CARTE: A Benchmark for Mapping Language Model Knowledge Across France

We introduce CARTE (Culturally Anchored Regional-Territorial Evaluation), a multiple-choice benchmark for evaluating the ability of large language models (LLMs) to discriminate fine grained, geographically grounded and regionally differentiated knowledge within France. While prior benchmarks focus on national-level cultural understanding, they largely overlook intra-country variation and the need to distinguish between closely related regional contexts. CARTE addresses this gap by introducing 3,132 questions spanning the 13 metropolitan regions of France and covering 12 thematic domains, including culture, language, demographics, economy, environment, and mobility. Questions underwent four-stage validation: human review, LLM-as-a-judge, model-based difficulty calibration, and a second human review. We further introduce CARTE-LV, a subset targeting Linguistic Variation across French regions, enabling focused evaluation of language-related differences. We evaluate 32 open-weight LLMs of 1B to 30B parameters and three frontier API models across zero-, one-, and three-shot settings. Our experiments reveal performance disparities across regions and model scales, suggesting systematic gaps in pretraining coverage and limited robustness to intra-national variation.

==> tab_difficulty_levels.tex <==
\begin{table}[h]
\centering
% \color{red}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrr}
\toprule
\textbf{Difficulty level} & \textbf{Models correct} & \textbf{Classified} & \textbf{CARTE} \\
\midrule
Level 1 (Easy) & $\geq$ 80\% & 808 & 808 \\
Level 2 (Medium) & 40--80\% & 1,393 & 1,387 \\
Level 3 (Hard) & 10--40\% & 782 & 937 \\
Suspicious-hard & $<$ 10\% & 190 & -- \\
\quad validated by reviewers & & 149 & $\rightarrow$ Hard \\
\quad rejected by reviewers & & 41 & removed \\
\midrule
\textbf{Total} & & 3,173 & 3,132 \\
\bottomrule
\end{tabular}}
\caption{Difficulty calibration via aggregate 0-shot accuracy of the 32 open-weight models. Questions that fewer than 10\% of the models answered correctly were flagged as suspicious-hard and sent back to the human reviewers; the validated ones are labeled Hard in v1.2.}
\label{tab:difficulty_levels}
\end{table}


==> tab_main_results.tex <==
\begin{table*}[t!]
\centering
% \color{red}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llr ccccccccc c}
\toprule
\textbf{Model} & \textbf{Type} & \textbf{Params} & \multicolumn{3}{c}{\textbf{0-shot}} & \multicolumn{3}{c}{\textbf{1-shot}} & \multicolumn{3}{c}{\textbf{3-shot}} & \textbf{Overall} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12}
 & & & \textbf{Easy} & \textbf{Med} & \textbf{Hard} & \textbf{Easy} & \textbf{Med} & \textbf{Hard} & \textbf{Easy} & \textbf{Med} & \textbf{Hard} & \textbf{Avg} \\
\midrule
\multicolumn{13}{l}{\textit{French-specific LLMs}} \\[2pt]
Luciole-23B-Instruct & IT & 23.2B & \textbf{99.4} & \textbf{87.7} & 37.2 & \underline{99.1} & 86.2 & 38.7 & \textbf{99.3} & 86.3 & 40.3 & 75.6 \\
Luciole-8B-Instruct & IT & 8.1B & 98.5 & 79.2 & 32.0 & 98.1 & 78.8 & 33.3 & 98.4 & 81.2 & 36.2 & 70.8 \\
Gaperon-1125-8B-SFT & IT & 8.0B & 96.2 & 72.5 & 24.2 & 95.0 & 69.6 & 26.5 & 96.8 & 74.2 & 29.0 & 64.6 \\
Gaperon-1125-8B & Base & 8.0B & 96.2 & 68.0 & 25.5 & 96.4 & 70.7 & 25.3 & 97.9 & 75.9 & 28.3 & 64.5 \\
% Occiglot-7B-FR-EN-Instruct\textsuperscript{new} & IT & 7.2B & 97.8 & 74.7 & 20.1 & 98.1 & 74.0 & 19.4 & 97.0 & 73.5 & 22.4 & 64.2 \\
% Vigogne-2-13B-Instruct\textsuperscript{new} & IT & 13.0B & 91.6 & 52.7 & 19.4 & 94.2 & 59.3 & 20.3 & 94.4 & 61.5 & 20.9 & 55.8 \\
Claire-Mistral-7B-0.1 & Base & 7.2B & 87.0 & 44.9 & 18.9 & 96.3 & 61.1 & 21.9 & 95.8 & 64.0 & 23.6 & 55.5 \\
Lucie-7B-Instruct-v1.1 & IT & 6.7B & 93.2 & 59.2 & 14.2 & 92.7 & 57.0 & 19.6 & 92.9 & 60.9 & 20.0 & 55.5 \\
Vigogne-2-7B-Instruct & IT & 6.7B & 87.6 & 47.4 & 18.6 & 88.2 & 49.1 & 16.3 & 88.9 & 48.5 & 17.3 & 49.4 \\
Luth-LFM2-1.2B & IT & 1.2B & 85.5 & 46.6 & 20.2 & 82.7 & 47.1 & 22.2 & 82.5 & 47.2 & 23.5 & 48.9 \\
Luciole-1B-Instruct & IT & 1.3B & 76.6 & 38.1 & 19.1 & 80.4 & 44.4 & 18.8 & 81.6 & 45.0 & 17.5 & 44.9 \\
Vigogne-7B-Instruct & IT & 6.7B & 47.6 & 28.6 & 25.1 & 56.3 & 29.6 & 21.8 & 54.5 & 29.3 & 21.9 & 33.4 \\
Claire-7B-0.1 & Base & 6.9B & 27.5 & 20.0 & 20.6 & 23.5 & 20.8 & 20.2 & 22.4 & 19.5 & 21.3 & 21.4 \\
CroissantLLMChat-v0.1 & IT & 1.3B & 25.4 & 20.7 & 17.2 & 19.4 & 21.1 & 20.7 & 20.5 & 21.1 & 19.3 & 20.6 \\
% Gaperon-1125-1B-SFT\textsuperscript{new} & IT & 1.5B & 26.6 & 19.3 & 18.7 & 20.2 & 19.9 & 18.1 & 21.5 & 21.0 & 17.7 & 20.2 \\
\midrule
\multicolumn{13}{l}{\textit{European multilingual LLMs}} \\[2pt]
% EuroLLM-22B-Instruct-2512\textsuperscript{new} & IT & 22.6B & 98.8 & 84.5 & 33.3 & \underline{99.1} & 84.9 & 35.3 & \textbf{99.3} & 86.5 & 37.5 & 73.9 \\
% Mistral-Small-24B-Instruct-2501\textsuperscript{new} & IT & 23.6B & 97.9 & 81.5 & 33.2 & 97.4 & 81.1 & 33.5 & 96.3 & 80.0 & 36.2 & 71.1 \\
Mistral-Nemo-Instruct-2407 & IT & 12.2B & 98.5 & 79.0 & 27.2 & 98.5 & 82.6 & 31.9 & 98.0 & 84.0 & 33.2 & 70.8 \\
EuroLLM-9B-Instruct-2512 & IT & 9.2B & 99.0 & 78.6 & 20.5 & 98.9 & 81.4 & 25.4 & 99.0 & 80.7 & 25.9 & 68.2 \\
Occiglot-7B-EU5-Instruct & IT & 7.2B & 98.0 & 70.2 & 19.4 & 98.8 & 71.7 & 21.5 & 97.8 & 73.1 & 22.2 & 63.4 \\
Mistral-7B-v0.1 & Base & 7.2B & 98.8 & 65.7 & 17.1 & 98.0 & 68.4 & 19.9 & 96.7 & 68.9 & 19.3 & 60.8 \\
Mistral-7B-Instruct-v0.3 & IT & 7.2B & 98.3 & 66.3 & 16.8 & 96.5 & 65.8 & 17.6 & 95.8 & 65.7 & 14.2 & 59.0 \\
Mistral-7B-Instruct-v0.2 & IT & 7.2B & 94.7 & 61.4 & 14.4 & 93.4 & 57.6 & 14.3 & 92.5 & 59.1 & 14.7 & 54.7 \\
\midrule
\multicolumn{13}{l}{\textit{General multilingual LLMs}} \\[2pt]
% Gemma-4-31B-IT\textsuperscript{new} & IT & 31.3B & 97.9 & \textbf{87.7} & \textbf{55.1} & 98.9 & \underline{89.8} & \textbf{60.3} & 99.0 & \underline{90.5} & \textbf{62.2} & \textbf{82.7} \\
% Qwen3.5-27B\textsuperscript{new} & IT & 27.8B & \underline{99.3} & \underline{87.5} & \underline{45.1} & 99.0 & \textbf{89.9} & \underline{49.5} & \underline{99.1} & \textbf{90.6} & \underline{53.5} & \underline{79.9} \\
% Gemma-3-27B-IT\textsuperscript{new} & IT & 27.4B & 98.9 & 84.3 & 40.0 & 98.3 & 82.7 & 39.8 & 97.6 & 83.5 & 41.5 & 74.4 \\
Qwen3.5-9B & IT & 9.0B & \underline{99.3} & 82.2 & 33.0 & \textbf{99.3} & 83.2 & 35.3 & 99.0 & 83.3 & 37.2 & 72.8 \\
Gemma-3-12B-IT & IT & 12.2B & 98.8 & 79.5 & 32.7 & 97.9 & 78.7 & 33.1 & 97.6 & 79.8 & 34.5 & 70.4 \\
GLM-4.7-Flash & IT & 29.9B & 98.3 & 79.7 & 33.1 & 97.2 & 78.2 & 31.2 & 97.6 & 78.1 & 34.0 & 69.8 \\
Llama-3.1-8B-Instruct & IT & 8.0B & \textbf{99.4} & 77.6 & 25.1 & 98.5 & 77.5 & 26.5 & 98.3 & 78.0 & 27.0 & 67.7 \\
Qwen3.5-4B & IT & 4.2B & 97.4 & 76.7 & 27.3 & 96.3 & 75.3 & 26.3 & 96.8 & 73.0 & 27.6 & 66.3 \\
GLM-4-9B-0414 & IT & 9.4B & 98.8 & 72.5 & 25.6 & 98.5 & 72.6 & 29.6 & 97.4 & 75.3 & 28.5 & 66.2 \\
Gemma-4-E4B-IT & IT & 7.9B & 97.3 & 71.2 & 23.6 & 97.8 & 74.2 & 25.2 & 97.4 & 76.1 & 27.1 & 65.4 \\
Aya-Expanse-8B & IT & 8.0B & 99.0 & 70.4 & 24.4 & 96.5 & 67.4 & 26.0 & 97.0 & 69.1 & 26.6 & 63.4 \\
Gemma-4-E2B-IT & IT & 5.1B & 94.7 & 61.2 & 19.2 & 94.3 & 62.5 & 20.8 & 93.1 & 62.3 & 21.3 & 57.8 \\
GLM-4-9B-Chat & IT & 9.4B & 95.9 & 62.4 & 14.7 & 95.7 & 61.8 & 16.2 & 94.6 & 62.3 & 16.5 & 56.9 \\
Llama-3.2-3B-Instruct & IT & 3.2B & 93.2 & 54.5 & 14.9 & 91.6 & 52.8 & 15.6 & 93.3 & 54.3 & 15.4 & 52.3 \\
Gemma-4-E2B & Base & 5.1B & 79.8 & 39.9 & 19.3 & 92.7 & 54.1 & 21.1 & 93.4 & 59.8 & 23.5 & 52.0 \\
Llama-3.2-1B-Instruct & IT & 1.2B & 79.5 & 40.5 & 19.4 & 75.2 & 40.6 & 21.5 & 74.8 & 41.2 & 22.1 & 44.1 \\
BLOOMZ-3B & IT & 3.0B & 81.6 & 38.8 & 20.0 & 46.9 & 22.6 & 14.0 & 54.0 & 28.3 & 20.4 & 34.4 \\
\midrule
\multicolumn{13}{l}{\textit{Frontier API models}} \\[2pt]
Gemini 3.8 Flash & API & -- & 99.3 & 96.6 & 88.8 & 99.9 & 96.5 & 89.0 & 99.8 & 97.3 & 88.8 & 95.2 \\
GLM-5.3-Flash & API & -- & 99.4 & 92.1 & 69.8 & 99.3 & 90.9 & 67.6 & 99.0 & 90.1 & 68.6 & 86.5 \\
GLM-5.3 & API & -- & 99.5 & 92.2 & 68.5 & 98.5 & 90.1 & 65.0 & 99.3 & 90.8 & 62.3 & 85.4 \\
\bottomrule
\end{tabular}%
}
% \caption{Accuracy (\%) on \benchmark\ per difficulty tier and $k$-shot setting ($k \in \{0, 1, 3\}$) for the 32 open-weight models run locally, and whole-set accuracy of the frontier API models scored on their generated answer (3,173-question filtered set; no per-question responses, hence no tiers). Type: Base = pretrained checkpoint prompted raw, IT = instruction- or chat-tuned checkpoint prompted through its chat template. \textbf{Bold} and \underline{underline} denote the highest and second-highest values per column among the local models. \textit{Overall Avg} is the accuracy on the whole set, averaged over the three shot settings.}
\caption{Accuracy (\%) on \benchmark\ across difficulty tiers and $k$-shot settings ($k \in \{0, 1, 3\}$) for 32 locally run open-weight models, alongside the accuracy for frontier API models (3,173-question filtered set; tier breakdown unavailable). Type: Base = pretrained checkpoint prompted raw, IT = instruction- or chat-tuned checkpoint prompted via chat template. \textbf{Bold} and \underline{underline} denote highest and second-highest values per column among local models. \textit{Overall Avg} denotes whole-set accuracy averaged across shot settings.}
\label{tab:CARTE_results}
\end{table*}

